Sponsored Search Auction Design Beyond Single Utility Maximization

Auction design for the modern advertising market has gained significant prominence in the field of game theory. With the recent rise of auto-bidding tools, an increasing number of advertisers in the market are utilizing these tools for auctions. The diverse array of auto-bidding tools has made auction design more challenging. Various types of bidders, such as quasi-linear utility maximizers and constrained value maximizers, coexist within this dynamic gaming environment. We study sponsored search auction design in such a mixed-bidder world and aim to design truthful mechanisms that maximize the total social welfare. To simultaneously capture the classical utility and the value-max utility, we introduce an allowance utility model. In this model, each bidder is endowed with an additional allowance parameter, signifying the threshold up to which the bidder can maintain a value-max strategy. The paper distinguishes two settings based on the accessibility of the allowance information. In the case where each bidder's allowance is public, we demonstrate the existence of a truthful mechanism achieving an approximation ratio of $(1+\epsilon)$ for any $\epsilon > 0$. In the more challenging private allowance setting, we establish that a truthful mechanism can achieve a constant approximation. Further, we consider uniform-price auction design in large markets and give a truthful mechanism that sets a uniform price in a random manner and admits bounded approximation in expectation.

==> 40-private_old.tex <==
\section{Private Allowance}\label{sec:private}

This section considers the setting where the allowance information $\vgamma$ is private. 
Compared to the public allowance setting, this scenario extends beyond the single-parameter environment, introducing increased complexity and posing greater challenges. 
In~\cref{alg:public}, the payment of bidder~$i$ is significantly dependent on the allowance $\gamma_i$. Such a strong correlation between the payment rule and $\vgamma$ indicates that when $\gamma_i$ becomes private, a bidder could benefit from misreporting a lower allowance.


% In~\cref{xxx}, the payment of bidder $i$ relies highly on allowance $\gamma_i$. 
% Such a highly $\vgamma$-related payment rule indicates that when $\gamma_i$ becomes private, the bidder could benefit from misreporting a lower allowance. 

To handle this issue, we explore \emph{$\vgamma$-independent} mechanisms, where both the allocation and payment rules are independent of the allowance profile of bidders, and show the following.

\begin{theorem}\label{thm:private}
    In the private allowance setting, there exists a $\vgamma$-independent mechanism which is truthful and $O(k^{2/3})$-approximation, where $k$ is the number of slots. 
\end{theorem}

To gain algorithmic intuition and streamline the analysis, we begin by considering the simplest case where $k=1$. Even in the presence of only one slot, developing a truthful and $\vgamma$-independent mechanism is not a trivial task.

\subsection{Single-Slot Auction}\label{subsec:private_single}

In this subsection, we consider the single-slot environment. Without loss of generality, assume that the slot's CTR is~$1$. Given our aim for a truthful mechanism, the auction must be truthful for any quasi-linear utility maximizer, i.e., the bidder with $\gamma_i=0$. For this type of bidders, Myerson’s Lemma~\cite{DBLP:journals/mor/Myerson81} dictates that the allocation rule must be monotone, and the payment rule is unique for a monotone allocation. Specifically, a bounded approximation mechanism should allocate the slot to one of the highest bidders and charge her the threshold bid.


Since we target a $\vgamma$-independent mechanism, we have to treat bidders as if they do not disclose their allowance profiles. Consequently, we are unable to distinguish whether a bidder employs quasi-linear utility or not. In light of this, to maintain truthfulness and a bounded approximation ratio, the classical second-price mechanism seems the most viable choice, where the highest bidder wins (with ties broken arbitrarily) and is charged the second-highest bid.


We examine the truthfulness of the second-price auction for bidders with $\gamma_i > 0$. Fortunately, due to the constraint $p_i \leq v_i\alpha_j$, these bidders are truthful in most cases, except in situations involving multiple highest bidders. When there is more than one highest bidder, quasi-linear utility maximizers have no incentive to lie because their utilities, whether they obtain the slot or not, consistently amount to~$0$. However, the scenario differs for other types of bidders. Upon securing the slot, they gain a non-zero utility, leading to a potential misreport of a higher bid to obtain the slot while paying an amount that adheres to the constraint. To tackle this challenge, we employ a scaling technique. The mechanism is described in~\cref{alg:private_single} and we show the following. % the details of which are outlined in~\cref{xxx}.


\begin{algorithm}[tb]
   \caption{\; $\vgamma$-Independent Single-Slot Auction}
   \label{alg:private_single}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} bids $\cB=\{b_i\}_{i\in [n]}$ and parameter $\epsilon>0$.
   \STATE {\bfseries Output:} allocation $\Pi$ and payment $\cP$.
   \STATE Initialize $\pi_i\leftarrow 2$ (the dummy slot) and $p_i\leftarrow 0 $, $\forall i\in [n]$.
   \FOR{each bidder $i\in [n]$}
   \STATE {\color{gray} /* Round $b_i$ down slightly such that it is an exponential multiple of $(1+\epsilon)$. */}
   \STATE Set $\barb_i=(1+\epsilon)^{\lfloor \log_{1+\epsilon} b_i \rfloor}$.
   \ENDFOR
   \STATE Use $\cS$ to denote the set of bidders with the highest $\barb$.
   \IF{ $|\cS| > 1$}
   \STATE {\color{gray} /* Break ties in a fixed manner. */}
    \STATE Let $k$ be the smallest index in $\cS$. 
    %the highest (rounded) bid and $b'_\ell$ be the second-highest one.
    \STATE Set $\pi_k \leftarrow 1$ and $p_k\leftarrow \barb_k$.
    \ELSE
    \STATE Let $\barb_k$ be the highest (rounded) bid and $\barb_\ell$ be the second-highest.
    \STATE Set $\pi_k \leftarrow 1$ and $p_k \leftarrow (1+\epsilon)\cdot \barb_\ell$.
   \ENDIF
   \STATE \textbf{return} $\Pi=\{\pi_i\}_{i\in [n]}$ and $\cP=\{p_i\}_{i\in [n]}$.
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:private_single}
    For any $\epsilon >0 $,~\cref{alg:private_single} is truthful and obtains an approximation ratio of $(1+\epsilon)$.
\end{theorem}

\begin{proof}
    We begin by analyzing the truthfulness of the mechanism. 
    If bidder $i$ can win the auction with a truthful bid $b_i=v_i$, she obtains a non-negative utility: regardless of whether $|\cS|$ is $1$ or greater, the payment is always at most the private value. 
    Consequently, she has no incentive to lie because the allocation is monotone and the payment does not rely on $b_i$. 
    
    In the case that bidder $i$ loses the game with a truthful bid, we have $\barb_i\leq \barb_k$, where bidder $k$ is the winner.
    Clearly, the only chance to potentially increase the utility is by misreporting a higher bid $b_i'$ that enables her to win. If $\barb_i< \barb_k$, bidder $i$ would violate the payment constraint upon winning: 
    \[p_i \geq \barb_k \geq (1+\epsilon)\cdot \barb_i > b_i=v_i.\]
    If $\barb_i = \barb_k$, the bidder loses the game due to the fixed tie-breaking. Therefore, to obtain the slot, the misreported bid must satisfy $\barb_i' \geq (1+\epsilon)\cdot \barb_k$, which also breaches the constraint as now $|\cS'|=1$ and the payment becomes
    \[ p_i = (1+\epsilon)\cdot \barb_k = (1+\epsilon)\cdot \barb_i > b_i=v_i. \]

    The proof of the approximation ratio is straightforward. Given that the winner $k$ has the highest $\barb_k$, any other bidder's value is at most $(1+\epsilon)\cdot v_k$. As the single-slot auction has $\opt=\max_{i\in [n]}v_i$, the mechanism is $(1+\epsilon)$-approximation.
    
    %The approximation ratio is easy to prove. Since the winner $k$ has the highest $\barb_k$, any other bid is at most $(1+\epsilon)b_k$, implying that the mechanism is $(1+\epsilon)$-approximation.
    
\end{proof}



%We examine the truthfulness of the VCG mechanism for the bidders with $\gamma_i >0$. Fortunately, due to the constraint that $p_i\leq v_i\alpha_j$, they are truthtellers in most cases, except the case that there are multiple highest bidders. For quasi-linear utility maximizers, they do not have the incentive to lie because whether they obtain the slot or not, their utilities are always $0$, there is no difference. However, the thing is different for other types of bidders. When they obtain the slot, they has a non-zero utility, thus, they may misreport a higher bid, obtaining the slot while paying the money that does not violate the constraint. To address this challenge, we employ a scaling technique. The mechanism is described in~\cref{xxx}.  


%Suppose that we allocate the slot to one of the highest bidders and use the second-price payment rule 

%Ensuring $\vgamma$-independence in the mechanism, 
% In this subsection, we consider the single-slot environment. Since we target a truthful mechanism, the mechanism must be truthful for any quasi-linear utility maximizer $\gamma_i=0$. According to Myerson’s Lemma~\cite{xxx}, the allocation rule should be monotone and the payment rule is unique --- that is, a bounded approximation mechanism should assign the slot to one of the highest bidders and charge her the second price. 
% Since the mechanism is required to be $\vgamma$-independent, we can pretend that bidders do not report their allowance profile and thus, we cannot distinguish whether a bidder uses quasi-linear utility or not. Thus, to guarantee truthfulness, the second-price payment rule is the only choice. 




%Clearly, to obtain a bounded approximation ratio, the mechanism has to allocate the slot to the top bidders (with high probability). The critical part is the design of the payment rule. Since the mechanism needs to be $\vgamma$-independent, the payment rule should make both the quasi-linear utility maximizers $\gamma_i=0$ and the value maximizers $\gamma_i=\infty$ truthful. According to Myerson’s Lemma~\cite{xxx}, the payment function is unique
%Since we focus on $\vgamma$-independent mechanisms, 

\cref{thm:private_single} proves a constant approximation for single-slot auction. This result can further be extended to the multiple-slot setting. Specifically, if there exists a bidder making a significant contribution to the optimal social welfare $\opt$, we can choose to auction only the first slot and then apply~\cref{alg:private_single} to achieve a bounded approximation ratio:

\begin{corollary}\label{cor:private_single}
    For the multiple-slot setting, if there exists a bidder $i$ with $v_i \cdot \alpha_1 \geq \frac{\opt}{\rho} $ for some $\rho \geq 1$, ~\cref{alg:private_single} is truthful and obtains $\rho \cdot (1+\epsilon)$ approximation.
\end{corollary}

%f there exists a bidder having a great  contribution on $\opt$, we can directly sell the first slot, view the auction as a single-slot auction, and employ~\cref{alg:private_single}. 


\subsection{Large Market Auction}

\cref{cor:private_single} gives a bounded approximation for the scenario where $\max_{i\in [n]}v_i \cdot \alpha_1 \geq \frac{\opt}{\rho} $. This subsection addresses the converse scenario – the large market case, where $\max_{i\in [n]}v_i \cdot \alpha_1 < \frac{\opt}{\rho}$. In a large market, no bidder or slot dominates.
In addition, we also assume, w.l.o.g., that $\rho$ is sufficiently large, e.g. $\rho \geq 36$.
Consequently, we can leverage the random sampling technique to develop a truthful mechanism with a bounded approximation ratio due to the following concentration lemma:

\begin{lemma}[~\cite{DBLP:journals/mor/ChenGL14}]\label{lem:concen}
    Let $a_1\geq a_2 \geq ... \geq a_\ell$ be positive real numbers, such that the sum $a=a_1+...+a_\ell$ satisfies $a_1 < a/36$. We select each number $a_1,...,a_\ell$ independently at random with probability $1/2$ each and let $b$ be the random variable equal to the sum of the selected numbers. Then
    \[ \Pr\left[\frac{a}{3} < b < \frac{2a}{3}\right] \geq \frac{3}{4}.  \]
\end{lemma}




\begin{algorithm}[tb]
   \caption{\; $\vgamma$-Independent Large Market Auction}
   \label{alg:private_large}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} bids $\cB=\{b_i\}_{i\in [n]}$, CTRs $\valpha=\{\alpha_j\}_{j\in [k]} $ and parameter $\beta \in (0,1)$.
   \STATE {\bfseries Output:} allocation $\Pi$ and payment $\cP$.
   \STATE Initialize $\pi_i\leftarrow k+1$ (the dummy slot) and $p_i\leftarrow 0 $, $\forall i\in [n]$.
   \STATE Pick the minimum index $t\in [k]$ such that $\sum_{j\in [t]}\alpha_j \geq \beta \cdot \sum_{j\in [k]}\alpha_j $.
   \STATE Randomly divide all the bidders with equal probability into set $\cS_1$ and $\cS_2$; subsequently, also with equal probability,  designate one of $\{ \cS_1, \cS_2 \}$ as the pricing benchmark set $\cL$ and the other as the target bidder set $\cR$.
   \STATE Define the market price $Z$ to be the $t$-th highest bid in $\cL$; if $|\cL|<t$, $Z$ is $0$.
   \STATE Arrange the bidders in set $R$ in an arbitrarily fixed order. As each bidder $i$ arrives, offer all remaining slots to her at a unit price of $Z$ and allow her to select the most profitable slot $j$: $\pi_i \leftarrow j$ and $p_i \leftarrow Z \cdot \alpha_j$. 
   \STATE \textbf{return} $\Pi=\{\pi_i\}_{i\in [n]}$ and $\cP=\{p_i\}_{i\in [n]}$.
\end{algorithmic}
\end{algorithm}

We describe the mechanism in~\cref{alg:private_large}. Initially, the mechanism randomly partitions all bidders into two subsets $\cS_1$ and $\cS_2$, each with an equal probability. In this procedure, both $\cS_1$ and $\cS_2$ can be viewed as generated by selecting each bidder independently at random with probability $1/2$ each. Due to~\cref{lem:concen}, we have the following:

\begin{lemma}\label{lem:subopt}
Use  $\opt(\cS_1)$, $\opt(\cS_2)$, and $ \opt$ to respectively represent the social welfares obtained exclusively by auctioning bidders in $\cS_1$, exclusively by auctioning bidders in $\cS_2$, and by auctioning all bidders in $[n]$. Under the large market assumption, we have 
\[\opt(\cS_1), \opt(\cS_2) \geq \frac{1}{3}\opt\] with probability at least $3/4$. 
    %Use $ \opt$, $\opt(\cS_1)$, and $\opt(\cS_2)$ to denote the optimal social welfares achieved through auctions involving all bidders, exclusively those in $\cS_1$, and exclusively those in $\cS_2$, respectively.
\end{lemma}

\begin{proof}
    Consider the allocation $\Pi^*$ in the optimal solution when auctioning all bidders in $[n]$. According to the definition of social welfare, we have
    \[ \sum_{i\in[n]} v_i\cdot \alpha_{\pi^*_i} = \opt. \]
    Due to the large market assumption, for any bidder $i\in [n]$
    \[ v_i\cdot \alpha_{\pi^*_i} < \frac{\opt}{36}. \]

    Both $\cS_1$ and $\cS_2$ can be viewed as generated by selecting each bidder independently at random with probability $1/2$ each. Thus, by~\cref{lem:concen},  
    \begin{equation}\label{eq:concen1}
        \Pr\left[ \frac{\opt}{3} < \substack{\sum\limits_{i\in\cS_1} v_i\cdot \alpha_{\pi^*_i} \\[1ex] \sum\limits_{i\in\cS_2} v_i\cdot \alpha_{\pi^*_i} } < \frac{2\opt}{3} \right] \geq \frac{3}{4}. 
    \end{equation}

    Observing that $\{\pi^*_i\}_{i\in \cS_1}$ is a feasible solution in the scenario that auctioning $\cS_1$, we have
    \begin{equation}\label{eq:concen2}
        \opt(\cS_1) \geq \sum\limits_{i\in\cS_1} v_i\cdot \alpha_{\pi^*_i}.
    \end{equation}
    Similarly,
    \begin{equation}\label{eq:concen3}
        \opt(\cS_2) \geq \sum\limits_{i\in\cS_2} v_i\cdot \alpha_{\pi^*_i} .
    \end{equation}

    Combining~\cref{eq:concen1},~\cref{eq:concen2} and~\cref{eq:concen3} completes the proof.
    
\end{proof}


Built on~\cref{lem:subopt}, we prove the following theorem. 
\begin{theorem}\label{thm:large_market}
    Under the large market assumption that $ \max_{i\in [n]}v_i \cdot \alpha_1 < \frac{\opt}{\rho} $, ~\cref{alg:private_large} is truthful and obtains an expected social welfare at least $\frac{3}{8} \cdot \frac{\beta}{1-\beta} \cdot \left(\frac{\rho}{3k} - \beta \right)  \cdot \opt  $, where $k$ is the number of slots.
\end{theorem}


 
\begin{proof}

The proof of truthfulness is straightforward. For bidders in $\cL$, they will not be assigned anything, and therefore, misreporting their information cannot improve the utilities; while for bidders in $\cR$, they are also truthtelling because their reported information determines neither the arrival order nor the market price.

Now we analyze the approximation ratio. We first give a lower bound of the expected objective $\alg$ achieved by~\cref{alg:private_large} and then establish the relationship between the lower bound and $\opt$. 

Use $Z_1$ and $Z_2$ to denote the $t$-th highest bid among bidders in $\cS_1$ and $\cS_2$, respectively. Supposing that $Z_1\leq Z_2$, if the unit price of slots is set to be $Z_1$, at least $t$ bidders in $\cS_2$ can afford the cost. Hence, in our mechanism, with a probability of $1/2$, there are at least $t$ bidders in $\cR$ purchasing slots. According to the definition of $t$, we obtain a lower bound of our mechanism's objective value:
\begin{equation}\label{eq:private_lower_bound}
    \begin{aligned}
        \E\left[ \alg \right] & \geq \frac{1}{2}\cdot \sum_{j\in [t]} \alpha_j \cdot \E\left[\min\left\{ Z_1, Z_2 \right\}\right] \\
        & \geq \frac{\beta}{2} \cdot \valpha \cdot \E\left[\min\left\{ Z_1, Z_2 \right\}\right],
    \end{aligned} .
\end{equation}
where we abuse the notion slightly and let $\valpha := \sum_{j\in [k]} \alpha_j$.

Next, we relate the lower bound to $\opt$. Consider the price benchmark set $\cL$. Denote by $V_{max}:=\max_{i\in[n]} v_i$ the maximum private value. Since $Z$ is the $t$-th highest bid, we obtain an upper bound of $\opt(\cL)$ by replacing all bids greater than $Z$ with $V_{max}$ and all bids less than $Z$ with $Z$:
\begin{equation*}
    \begin{aligned}
          \left(\beta \cdot V_{max} + (1-\beta)\cdot Z\right) \cdot \valpha \geq \opt(\cL) \;, 
    \end{aligned}
\end{equation*}

\cref{lem:subopt} implies that with probability at least $3/4$, $\opt(\cL) \geq \frac{1}{3}\opt$. Due to the large market assumption that $\opt > \rho \cdot  V_{max} \cdot \alpha_1$, 
\begin{equation}\label{eq:private_large_opt}
    \begin{aligned}
       \left(\beta \cdot V_{max} + (1-\beta)\cdot Z\right) \cdot \valpha & \geq \frac{1}{3} \cdot \opt \\
       \left(\beta \cdot V_{max} + (1-\beta)\cdot Z\right) \cdot \valpha & \geq \frac{1}{3}\cdot \rho \cdot  V_{max} \cdot \alpha_1 \\
       \beta \cdot V_{max} + (1-\beta)\cdot Z & \geq \frac{1}{3}\cdot \rho \cdot  V_{max} \cdot \frac{\alpha_1}{\valpha} \\
       \beta \cdot V_{max} + (1-\beta)\cdot Z  & \geq \frac{1}{3}\cdot \rho \cdot  V_{max} \cdot \frac{1}{k} \\
       Z & \geq \frac{1}{1-\beta} \cdot \left(\frac{\rho}{3k} - \beta \right)\cdot V_{max}
    \end{aligned}.
\end{equation}

Note that~\cref{eq:private_large_opt} holds for both $Z_1$ and $Z_2$ with probability at least $3/4$. Combining it with~\cref{eq:private_lower_bound}, we complete the proof:
\begin{equation*}%\label{eq:private_lower_bound}
    \begin{aligned}
        \E\left[ \alg \right] & \geq \frac{\beta}{2} \cdot \valpha \cdot \frac{3}{4} \cdot  \frac{1}{1-\beta} \cdot \left(\frac{\rho}{3k} - \beta \right)\cdot V_{max} \\
        & \geq \frac{3}{8} \cdot \frac{\beta}{1-\beta} \cdot \left(\frac{\rho}{3k} - \beta \right) \cdot \opt
    \end{aligned}. 
\end{equation*}




% Since the mechanism designates $\cL$ and $\cR$ randomly, at least $t$ bidders in $\cR$ afford the unit price of $Z$ with probability at least $1/2$. 

    
\end{proof}

By setting $\beta = 1-\sqrt{1-\frac{\rho}{3k}}$, we get the best approximation:
\begin{equation}\label{eq:private_large_final}
    \E [\alg] \geq \frac{3}{8} \left( 1-\sqrt{1-\frac{\rho}{3k}} \right)^2 \cdot \opt .
\end{equation}


%considers the other side --- the large market case where $\max_{i\in [n]}v_i \cdot \alpha_1 < \frac{\opt}{\rho} $. In the large market, there is no dominant bidder and slot. Thus, we can employ the random sampling technique to obtain a truthful mechanism with a bounded approximation ratio. The mechanism is described in~\cref{xxx}.

\subsection{Final Mechanism}

This subsection builds on~\cref{alg:private_single} and~\cref{alg:private_large} to give the final mechanism. Essentially, it is a random combination of the two mechanisms. See~\cref{alg:private_final}.  

\begin{algorithm}[tb]
   \caption{\; $\vgamma$-Independent Auction}
   \label{alg:private_final}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} bids $\cB=\{b_i\}_{i\in [n]}$, CTRs $\valpha=\{\alpha_j\}_{j\in [k]} $ and parameter $\rho \in (1,k)$.
   \STATE {\bfseries Output:} allocation $\Pi$ and payment $\cP$.
   \BEGIN{With probability of $1/2$}
   \STATE Run~\cref{alg:private_single} to sell the first slot.
   \ENDBEGIN
   \BEGIN{With probability of $1/2$}
   \STATE Run~\cref{alg:private_large} with parameter $\beta = 1-\sqrt{1-\frac{\rho}{3k}}$.
   \ENDBEGIN
   \STATE \textbf{return} $\Pi=\{\pi_i\}_{i\in [n]}$ and $\cP=\{p_i\}_{i\in [n]}$.
\end{algorithmic}
\end{algorithm}

\begin{proof}[Proof of~\cref{thm:private}]
    We show that~\cref{alg:private_final} is truthful and $O(k^{2/3})$-approximation. The mechanism randomly picks one procedure and execute it. Due to the truthfulness guarantee of each procedure,~\cref{alg:private_final} is truthful. 

    Use $\alg_1, \alg_2$ to denote the social welfares obtained by the two procedures, respectively. Since each procedure is executed with probability $1/2$, the final mechanism has
    \[ \E[\alg] = \frac{1}{2}\cdot \left( \alg_1 + \E[\alg_2] \right). \]

    When the instance satisfies the large market assumption, due to~\cref{thm:large_market}, 
    \[ \E[\alg_2] \geq \frac{3}{8} \left( 1-\sqrt{1-\frac{\rho}{3k}} \right)^2 \cdot \opt; \]
    otherwise, the objective value of the first procedure is bounded by~\cref{cor:private_single}:
    \[ \alg_1 \geq \frac{1}{\rho \cdot (1+\epsilon)}  \cdot \opt. \]

    Combining the above two cases, we have
    \[\frac{\E[\alg]}{\opt} \geq \min\left\{\frac{1}{2\rho \cdot (1+\epsilon)} , \frac{3}{16} \left( 1-\sqrt{1-\frac{\rho}{3k}} \right)^2  \right\}  . \]
    Finally, setting $\rho = O(k^{2/3})$ proves the claimed ratio.
    
    
\end{proof}

% The entire mechanism  

% %The case is even non-trivial when there is only one slot. 

% It is even non-trivial for the case where there is only one slot. 

%To handle this issue, we employ the random sampling technique. 






\iffalse
\section{Random Sampling on Private Value and Constraint}
    
    \begin{algorithm}[tb]
       \caption{Random Sampling on Private Value and Constraint}
       \label{alg:Algorithm3}
    \begin{algorithmic}
        \STATE {\bfseries Input:} The CTR X =  $\{ x_k \} _{k \in [m] }$ of m slots, the reported value V = $\{v_i\} _{i \in [n]}$ and the constraint C = $\{ c_i \} _{i \in [n] }$ of all bidders 
        \STATE {\bfseries Output:} The allocation and payment of all bidders
        \STATE Initialize $\pi_k = 0 \ \forall k \in [m],\ a_i = 0,p_i = 0 \ \forall i \in [n]$
        \STATE Compute offline maximum social welfare SW = $\sum_{i=1}^m x_i v_i$
        \IF{$x_m v_m \ge \frac{1}{12}SW$}
            \STATE Allocate slot 1 to bidder 1, i.d., $\pi_1 = 1, a_1 = 1$
        \ELSE
            \STATE Randomly divide all the bidders with equal probability into 2 sets S and R
            \STATE \qquad //set the reserve price based on the bid in S
            \STATE Select the top m bidders by their bid in S and R respectively, use $\{v_i^S\}_{i \in [m]}$ and $\{v_i^R\}_{i \in [m]}$ to denote the i-th highest bid in S and R. 
            %\STATE Set reverse price $p_k \leftarrow \frac{1}{2} v_k^S \ \forall \in [m]$
            \STATE \qquad // Allocate all slots to bidders in R
            \FOR{$i=1$ {\bfseries to} $m$}
            \STATE slot i $\leftarrow$ bidder $i^R$ in R ,$\ i.d. \pi_i = i^R, a_i^R = i $, where $i^R \in R $, with value $v_i^R$
            \STATE $p_i^R \leftarrow \frac{1}{2} v_k^S$
            \ENDFOR
        \ENDIF
    \end{algorithmic}
    \end{algorithm}
    
    In this section and subsequent sections, we will discuss a new model wherein the budget and constraints of agents are private.
    Before we introduce the final mechanism, to streamline the analysis, we first introduce an auxiliary mechanism \cref{alg:Algorithm3}, which is a random sampling idea.This mechanism is constant-approximate but not truthful, and then we show it can be altered to a truthful mechanism by losing only a constant factor on the approximation ratio.
    
    \textbf{Theorem 3.} \cref{alg:Algorithm3} obtains a constant approximation ratio for social welfare, and? for the auctioneer's revenue.
    
    \textit{Proof.} Be continue.....

    Be continue.....



\fi

==> 41-private-alter.tex <==
\section{Another Private Mechanism with Constant Approximation ratio}\label{sec:private2}
% 这一部分放在40-private里面更好，因为最后还是需要它跟只分配一个机制的混合使用

\subsection{An auxiliary mechanism in large market auction}
% 整理思路用，大概不用放进去
\begin{algorithm}[tb]
   \caption{\; (Auxiliary) Large Market Auction - 2}
   \label{alg:aux_private_large2}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} bids $\cB=\{b_i\}_{i\in [n]}$, CTRs $\valpha=\{\alpha_j\}_{j\in [k]} $.
    \STATE {\bfseries Output:} allocation $\Pi$.
    \STATE Randomly divide all the bidders with equal probability into set $\cS_1$ and $\cS_2$, sort them by their bids in descending order,and use $v_i$ and $w_i$ to denote the i-th highest bid in $\cS_1$ and $\cS_2$ respectively.
    \STATE Subsequently, with equal probability, designate one of $\{ \cS_1, \cS_2 \}$ as the pricing benchmark set $\cL$ and the other as the target bidder set $\cR$.
    \STATE Initialize $\pi_i\leftarrow k+1$ (the dummy slot) $\forall  i \in \cR$.
    \STATE The allocation rule: $\pi_i \leftarrow i$ if $w_i \ge v_i$ $\forall i \in [k]$. Namely, One in $\cR$ can take the slot only if her bid is not less than the counterpart with same index in $\cL$.
    \STATE \textbf{return} $\Pi=\{\pi_i\}_{i\in [n]}$ 
\end{algorithmic}
\end{algorithm}

Before introducing the final mechanism with a constant approximation ratio for Large Market Auction, for the sake of clarity, we present a auxiliary mechanism in \cref{alg:aux_private_large2}. We set aside its payment rule and focus only on its allocation rule. 
Although \cref{alg:aux_private_large2} is not truthful, we can then show it can be altered to a truthful mechanism  and it will serve as a bridge for our analysis between the $\opt$ and the final mechanism \cref{alg:private_large2}.

We introduce a lemma based on \cref{lem:concen} to proof its approximation ration, and the proof of \cref{lem:1/2} is deferred to \cref{sec:Appendix}.
\begin{lemma}\label{lem:1/2}
    Let $a_1\geq a_2 \geq ... \geq a_{2\cdot \ell}$ be positive real numbers, such that the sum $a=a_1+...+a_{2 \cdot \ell}$ satisfies $a_1 < a/36$. We select each number $a_1,...,a_\ell$ independently at random with probability $1/2$ into two sets, w.l.o.g., denote as $B = \{b_i\}_{i \in [\ell]}$ and $C = \{c_i\}_{i \in [\ell]}$ and both are rearranged in descending order.
    Then \[ \Pr\left[\frac{a}{3} < \sum\limits_{i \in [\ell]} \min \{b_i, c_i\}  < \frac{2a}{3}\right] \geq \frac{1}{2}.  \]
\end{lemma}

\begin{theorem}\label{thm:aux}
    The approximation ratio of \cref{alg:aux_private_large2} is at least $\frac{1}{12}$.
\end{theorem}
\begin{proof}
    
   % 其实我感觉之前用到的那个lemma那里有点不严谨，因为准确一点应该是有2l个数，里面取最大2k个数，和为a。然后把2l个数随机分成两个长度为l的list B和C。分别取B和C里面前k大的数的和，为b、c。有Pr[1/3a< b,c <2/3a] > 3/4 才对.就是似乎需要用到之前提到过的单价单调性和socialwelfare 单调性，不过大概意思应该没问题
    % 感觉这个事件出现太多次了，不知道放在哪里。。
    Based on \cref{lem:concen} and \cref{lem:1/2}, we prove \cref{thm:aux} as follows.

    Note that if we designate $\cS_2$ as $\cR$, the social welfare is $\alg_{aux}[\cS_2] \coloneqq \sum\limits_{i \in [k], w_i>v_i} v_i \cdot \alpha_i$.
    That is due to bidder i in $\cR$ who gets a slot only if her value exceeds the value of the bidder in $\cL$ in corresponding with index. Therefore, the social welfare is at least the total price of the slots they purchase.

    Similarly, when we designate $\cS_1$ as $\cR$,  the social welfare is $\alg_{aux}[\cS_1] \coloneqq \sum\limits_{i \in [k], v_i>w_i} w_i \cdot \alpha_i$.
    Compute its expectation:
    \begin{equation}\label{eq:optdefine}
        \begin{aligned}
                    \E[\alg_{aux}] 
                    &= \Pr[Assign\ \cS_2\ to\ \R] \cdot \alg_{aux}[\cS_2] + \Pr[Assign\ \cS_1\ to\ \R] \cdot \alg_{aux}[\cS_1] \\
                    &= \frac{1}{2} \cdot \E[\sum\limits_{i \in [k]} \min \{w_i\alpha_i, v_i \alpha_i\}]  \\
                    &\ge \frac{1}{2} \cdot \frac{1}{2} \cdot \frac{1}{3} \cdot OPT  = \frac{1}{12} \opt
        \end{aligned}
    \end{equation}
    where $\opt$ is the optimal social welfare $\opt = \sum\limits_{i \in [k]} b_i\cdot\alpha_i$.
    The third equation holds because we assume this setting to be a Large Market Auction, in where each bidder's contribution to social welfare is limited. Therefore, completing the proof.
\end{proof}


\subsection{honnban}

This subsection states a truthful mechanism with a constant approximation, which adapts similar techniques with \cref{alg:aux_private_large2}. The mainly difference is that, we price each slot discriminatively based on the bid of the corresponding bidder, and we let each bidder in $\cR$ come in an arbitrarily fixed order to select her favorite slot. 

\begin{algorithm}[tb]
   \caption{\; $16$-approximation Large Market Auction - 2}
   \label{alg:private_large2}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} bids $\cB=\{b_i\}_{i\in [n]}$, CTRs $\valpha=\{\alpha_j\}_{j\in [k]} $.
   \STATE {\bfseries Output:} allocation $\Pi$ and payment $\cP$.
    \STATE Randomly divide all the bidders with equal probability into set $\cS_1$ and $\cS_2$, sort them by their bids in descending order,and use $v_i$ and $w_i$ to denote the i-th highest bid in $\cS_1$ and $\cS_2$ respectively.
    \STATE Subsequently, with equal probability, designate one of $\{ \cS_1, \cS_2 \}$ as the pricing benchmark set $\cL$ and the other as the target bidder set $\cR$.
   \STATE Initialize $\pi_i\leftarrow k+1$ (the dummy slot) and $p_i\leftarrow 0 $, $\forall i\in \cR $.
   \STATE For each slot j in [k], set the price with unit price $up_j = \frac{1}{2} v_j$(maybe $w_i$).  
   \STATE Arrange the bidders in set $\cR$ in an arbitrarily fixed order. As each bidder $i$ arrives, allow her to select the most profitable slot $j$: $\pi_i \leftarrow j$ and $p_i \leftarrow up_j \cdot \alpha_j$. 
   \STATE \textbf{return} $\Pi=\{\pi_i\}_{i\in [n]}$ and $\cP=\{p_i\}_{i\in [n]}$.
\end{algorithmic}
\end{algorithm}



\begin{theorem}\label{thm:private_honnban}
    In the private allowance setting, under the large market assumption there exists a truthful $\vgamma$-approximation mechanism \cref{alg:private_large2}.
\end{theorem}

\begin{proof}
    
    Use $\opt(\cS_1) =  \sum\limits_{i \in [k]} v_i \alpha_i$ and  $\alg(\cS_1)$ to denote the optimal social welfare when considering only $\cS_1$ and  the social welfare of our solution when let $\cS_1$ as the target bidder set $\cR$, respectively. Similarly, $\opt(\cS_2) =  \sum\limits_{i \in [k]} w_i \alpha_i$ and $\alg(\cS_2)$ are defined the same as $\opt(\cS_1)$ and  $\alg(\cS_1)$, 
    Recalling \cref{lem:concen}, we have \[ \Pr\left[\frac{1}{3}\opt < \opt(\cS_1),\opt(\cS_2)  < \frac{2}{3} \opt \right] \geq \frac{3}{4}.\] where $\opt$ is defined the same as in \cref{eq:optdefine}.
    According to \cref{lem:1/2}, if we randomly divide all bidders into two group $\cS_1$ and $\cS_2$, then 
    \begin{equation}\label{eq:pi_orrurs}
        \Pr \left[ \frac   {1}{3}\opt < \sum\limits_{i \in [k]} \min \{w_i\alpha_i, v_i \alpha_i\}   < \frac{2}{3}\opt \right] \ge \frac{1}{2}
    \end{equation}
    
    we denote this event by $\mathbf{\Pi}$ for convenience, and the subsequent analysis is totally based on the occurrence of $\mathbf{\Pi}$. For the sake of convenience, expressions  $\mathbf{\Pi}$ in conditional probability are no longer displayed in the following analysis.
    
    Suppose that we designate $\cS_2$ as set $\cR$ and consider the behavior of each bidder i in $\cS_2$ with $w_i \le v_i$.
    % An intuitive but not accurate explanation is: Among two bidders with the same rank, if the one with lower value can obtain a slot, then if in the symmetric scenario, the other can obtain a slot, the latter also brings more social welfare than the former.
    Specifically, we distinguish the relationship between i and the index $j = \pi_i ,j \in [k+1]$ of the slot he purchases(the case she have not bought any slot is also considered), as the following 3 cases:
    \begin{enumerate}
        \item j = i in a numerical sense. Since bidder i have selected slot i, then the value of bidder i must be not less than the unit price for slot j, namely $w_i \ge up_i = \frac{1}{2} v_i$, Thus
            \begin{equation}\label{eq:case1}
                \frac{1}{2} v_i \cdot \alpha_i \le w_i \alpha_i =  w_i \alpha_j \quad \forall i \in \cS_2 ,j = \pi_i = i
            \end{equation}

 
            
        % 注意降序排序，j越小，代表东西越多
        \item j < i in a numerical sense. In such case bidder i purchases slot j with higher CTR $\alpha_j \ge \alpha_i$, also $w_i \ge up_j \ge up_i = \frac{1}{2} v_i$ holds. Thus,
            \begin{equation}\label{eq:case2}
                \frac{1}{2} v_i \cdot \alpha_i \le \frac{1}{2} v_j \cdot \alpha_j \le w_i \alpha_j \quad \forall i \in \cS_2 ,j = \pi_i > i
            \end{equation}
   
        
        
        \item j > i in a numerical sense. Then consider bidder i's utility, we have 
            \[ w_i \cdot \alpha_i - (up_i \cdot \alpha_i - \gamma_i)^+ = u_i\Big|_{j=i}  <   u_i'\Big|_{j>i} = w_i \cdot \alpha_j - (up_j \cdot \alpha_j - \gamma_i)^+. 
            \]
            We can assert that in such scenario her allowance must be exhausted if we allocate slot i to bidder i, otherwise she would have no reason to purchase a slot with a lower CTR since her payment does not matter. Thus, 
            \begin{equation*}\label{eq:prerequisite1}
                \begin{aligned}
                    w_i \cdot \alpha_i - up_i \cdot \alpha_i + \gamma_i 
                    & < w_i \cdot \alpha_j - (up_j \cdot \alpha_j - \gamma_i)^+ \\
                    & < w_i \cdot \alpha_j - (up_j \cdot \alpha_j - \gamma_i) \\
                    & = w_i \cdot \alpha_j - up_j \cdot \alpha_j + \gamma_i \\
                    w_i \cdot \alpha_i - \frac{1}{2}v_i \cdot \alpha_i 
                    & = w_i \cdot \alpha_i - up_j \cdot \alpha_j
                    < w_i \cdot \alpha_j 
                \end{aligned}
            \end{equation*}
            
            Recall that we only consider those bidders with $w_i \le v_i$ in $\cS_2$, we have
            \begin{equation}\label{eq:case3}
                \frac{1}{2}v_i \cdot \alpha_i  = v_i \cdot \alpha_i - \frac{1}{2}v_i \cdot \alpha_i  < w_i \cdot \alpha_i - \frac{1}{2}v_i \cdot \alpha_i  < w_i \cdot \alpha_j \quad \forall i \in \cS_2 ,j = \pi_i < i
            \end{equation}
    
    \end{enumerate}


    Synthesizing \cref{eq:case1}, \cref{eq:case2} and \cref{eq:case3}, summing both sides respectively, we can establish a lower bound between $\opt(\cS_1)$ and $\alg(\cS_2)$:
    \begin{equation}\label{eq:lb1}
        \begin{aligned}
            \frac{1}{2} \opt(\cS_1) &= \frac{1}{2}\sum\limits_{i \in [k]} v_i \alpha_i \\
            &= \frac{1}{2}\{\sum\limits_{i \in \cS_1, j = i}v_i \alpha_i + \sum\limits_{i \in \cS_1, j < i}v_i \alpha_i + \sum\limits_{i \in \cS_1, j > i}v_i \alpha_i\}\\
            &\le 
                \sum\limits_{i \in \cS_2, j = i}w_i \alpha_j + \sum\limits_{i \in \cS_2, j < i}w_i \alpha_j  + \sum\limits_{i \in \cS_2, j > i}w_i \alpha_j 
            \\
            &= \textcolor{red}{2} \cdot \alg(\cS_2 \Big| \mathbf{\Pi} )
        \end{aligned}
    \end{equation}
    %为什么是2不是3 是因为一个slot最多出现两次，如果完美比配达到opt就是1了，其实就算是3也不影响常数的近似比，但是我不知道怎么表达清楚只出现两次这个case。。。
   
    Due to we arbitrarily assign one of $\cS_1$ and $\cS_2$ as the target set $\cR$ with equally probability, we can similarly derive a lower bound between $\opt(\cS_2)$ and $\alg(\cS_1)$ when we let $\cS_1$ be $\cR$:
    \begin{equation}\label{eq:lb2}
        \begin{aligned}
            \frac{1}{2} \opt(\cS_2) \le 2 \cdot \alg(\cS_1 \Big| \mathbf{\Pi})
        \end{aligned}
    \end{equation}
    
    By aggregating \cref{eq:lb1}, \cref{eq:lb2} and \cref{lem:1/2}, when $\mathbf{\Pi}$ occurs, we have
    \begin{equation}
    \label{eq:shi_zai_shi_bu_xiang_qu_ming_zi_le}
        \begin{aligned}
            \frac{1}{3}\opt &\le \frac{1}{2}\opt(\cS_1) + \frac{1}{2} \opt(\cS_2) \\
            &\le 2 \cdot \alg(\cS_2 \Big| \mathbf{\Pi}) + 2 \cdot \alg(\cS_1 \Big| \mathbf{\Pi} ) = 4 \cdot \E[\alg \Big| \mathbf{\Pi}]
        \end{aligned}
    \end{equation}
     
 
    The last equation holds is because $\alg(\cS_1\Big|\mathbf{\Pi}) = \alg(\cS_2\Big|\mathbf{\Pi})$ since $\cS_1$ and $\cS_2$ is indifference in this mechanism.

    Combining \cref{eq:pi_orrurs} and \cref{eq:shi_zai_shi_bu_xiang_qu_ming_zi_le}: 
    \[
        \E[\alg] = \Pr[\mathbf{\Pi}] \cdot \ \E[\alg \Big| \mathbf{\Pi}]  + \Pr[\neg\mathbf{\Pi}] \cdot \ \E[\alg \Big| \neg\mathbf{\Pi}] > \frac{1}{2}\cdot \frac{1}{12} \opt + 0 = \frac{1}{24}\opt
    \]
    completes the proof.
    
    
\end{proof}



